Boosting vision transformers for image retrieval

Vision transformers have achieved remarkable progress in vision tasks such as image classification and detection. However, in instance-level image retrieval, transformers have not yet shown good performance compared to convolutional networks. We propose a number of improvements that make transformers outperform the state of the art for the first time. (1) We show that a hybrid architecture is more effective than plain transformers, by a large margin. (2) We introduce two branches collecting global (classification token) and local (patch tokens) information, from which we form a global image representation. (3) In each branch, we collect multi-layer features from the transformer encoder, corresponding to skip connections across distant layers. (4) We enhance locality of interactions at the deeper layers of the encoder, which is the relative weakness of vision transformers. We train our model on all commonly used training sets and, for the first time, we make fair comparisons separately per training set. In all cases, we outperform previous models based on global representation. Public code is available at https://github.com/dealicious-inc/DToP.

==> tex/related.tex <==
\section{Related work}
\label{sec:related}

In this section, we focus on work related to our high-level goal, that is, improving vision transformers for image retrieval. Work related to our particular ideas is discussed in \autoref{sec:design}.

\paragraph{Image retrieval based on convolutional networks}

Several studies in image retrieval~\cite{Gordo01, Kalantidis01, Weyand01, Weyand02, Radenovic01} are based on global descriptors. Common pooling methods are SPoC~\cite{Weyand02}, CroW~\cite{Kalantidis01}, R-MAC~\cite{Gordo01}, and GeM~\cite{Radenovic01}. More recently, attention-based methods are studied~\cite{Ng01,SCH01}. Alternative approaches are to use local descriptors to re-rank according to geometry~\cite{delf,cao2020unifying,Oriane} or build an aggregated representation~\cite{Giorgos, RITAC18}. The latter approaches have better performance but require more computational resources. It is common to have interaction between local and global feature extraction~\cite{cao2020unifying, yang2021dolg}.
%------------------------------------------------------------------------------

\paragraph{Vision transformers}

Starting with ViT~\cite{VIT}, vision transformers are being very actively studied in computer vision. Many recent studies~\cite{deit, twins, dvit, conformer, tokens, convit, Swin, rvt, levit, cait, tokenlabeling, tnt, sovit, patchvisiontransformer, att, cpe, vil, zhou2021ELSA, yuan2021incorporating, chen2021regionvit} have been shown effective, mostly on image classification but also on object detection~\cite{detr, Swin}.
Early models are mostly convolution-free; subsequently, several studies combine transformers with convolution~\cite{pit, coat, cvt, localvit, Visformer}. Self-supervised learning of transformers is emerging~\cite{dino, chen2021mocov3, sslswin}. We empirically investigate a large number of architectures on image retrieval and choose a hybrid ViT model as default.

%------------------------------------------------------------------------------

\paragraph{Transformer-based image retrieval}

Many transformer-based studies use models pre-trained on large scale datasets and apply them to downstream tasks such as object detection and segmentation. On image retrieval, there are only few studies. After initial off-the-shelf experiments~\cite{gkelios2021investigating}, the \emph{image retrieval transformer} (IRT)~\cite{IRT} has fine-tuned the model specifically for image retrieval~\cite{Radenovic01}. The self-supervised regime is examined in DINO~\cite{dino}. The \emph{re-ranking transformer} (RRT)~\cite{fwtan_instance_2021} uses a transformer to re-rank images by local features, while \emph{super-features}~\cite{superfeatures} aggregates local features by an iterative, transformer-inspired cross-attention mechanism;  but in both cases, the features are still obtained by a convolutional network. No study has achieved performance competitive with convolutional networks so far. In this work, we introduce a new approach to obtain a global image representation from a vision transfomer. We perform extensive experiments on several training sets and we show that our \ours outperforms convolutional networks, including local descriptors in certain cases.
